Differentially Private Heatmaps

We consider the task of producing heatmaps from users' aggregated data while protecting their privacy. We give a differentially private (DP) algorithm for this task and demonstrate its advantages over previous algorithms on real-world datasets. Our core algorithmic primitive is a DP procedure that takes in a set of distributions and produces an output that is close in Earth Mover's Distance to the average of the inputs. We prove theoretical bounds on the error of our algorithm under a certain sparsity assumption and that these are near-optimal.

==> exp-synth.tex <==
\section{Experimental Results on Synthetic Data}

In this section we present a few results on data that is synthetically generated.  We generate the  data by sampling from a uniform mixture of two-dimensional Gaussian distributions, while the mean and covariance matrix of each Gaussian is randomly generated. The number of Gaussians, their covariances, and the  number of samples from the mixture, are changed to control the sparsity of data.  
%We have generated synthetic data sets from sparsity $\sim 1\%$ to $\sim 75\%$. 
Throughout the experiments, we fix the number of users to 200, $\eps = 1$, and use $w = 20$.

We run two sets of experiments to demonstrate the effect of sparsity levels. In the first set of experiments, we fix the number of clusters to $20$. We then sample points from this Gaussian mixture until we reach different sparsity values. For each sparsity level, we generate 10 datasets. The experiment results are shown in \Cref{fig:sparsity-v-utility-20-clusters}. (Note that we bucketize the sparsity level.)

In the second set of experiments, we vary both the sparsity levels and the number of Gaussians in the mixture. Specifically, we use $5$ or $10$ Gaussians to produce low sparsity level $< 5\%$, $20$ clusters to produce mid-level sparsity like $\unsim 15\%$ and $\unsim 30\%$, and $80$ clusters to produce sparsity level like $\unsim 75\%$. 
%Other parameters, i.e. the variance of each Gaussian and the number of trials, remain the same as before. 
The results for this set of experiments are shown in \Cref{fig:sparsity-v-utility-varying-clusters}.

In both experiments, the rough trends are fairly similar: our algorithm's utility decreases as the sparsity level increases, wheres the baseline's utility increases. Upon closer inspection, however, the rate at which our algorithm's utility decreases is slower when we fixed the number of Gaussians. Indeed, this should be unsurprising: our guarantee is with respect to the best $k$-sparse approximation (in EMD), which remains roughly constant for the same mixture of Gaussians, regardless of the sparsity. As such, the utility does not decrease too dramatically if we keep the mixture distribution the same. On the other hand, when we also increase the number of Gaussians in the mixture, even the $k$-sparse approximation fails to capture it well\footnote{Note that while we do not choose $k$ explicitly, it is governed by the parameter $w$, which we fix to $20$ throughout.}, resulting in faster degradation in utility.

\begin{figure*}
\centering
\includegraphics[trim={0cm 0 0cm 0},clip,scale=0.275]{20clusters_dense_bin6.png}
\caption{Metrics averaged over 10 runs when varying the sparsity of the dataset; the number of Gaussians in the mixtures is kept constant at $20$ respectively. Shaded areas indicate 95\% confidence interval.%From left to right: Similarity, Pearson’s Correlation Coefficient, KL-divergence and EMD.
\label{fig:sparsity-v-utility-20-clusters}}
\end{figure*}

\begin{figure*}
\centering
\includegraphics[trim={0cm 0 0cm 0},clip,scale=0.275]{varing_clusters.png}
\caption{Metrics averaged over 10 runs when varying both the sparsity of the dataset and the number of Gaussians in the mixture; the number of Gaussians is increased from 5 to 10, 20, and 80. Shaded areas indicate 95\% confidence interval.%From left to right: Similarity, Pearson’s Correlation Coefficient, KL-divergence and EMD.
\label{fig:sparsity-v-utility-varying-clusters}}
\end{figure*}


==> proofs.tex <==
\section{Deferred Proofs}

\subsection{Proof of \Cref{lem:err-from-normalization}}

\begin{proof}[Proof of \Cref{lem:err-from-normalization}]
Let $\zeta = \|\bs - \hbs\|_{\emd}$; observe that $|\|\bs\|_1 - \|\hbs\|_1| \geq \zeta$. As a result, we have $\|\hbs\|_1 \in [n - \zeta, n + \zeta]$. Thus,
\begin{align*}
\|\hbs/n - \hba\|_{\emd} 
&\leq \|\hbs\|_{\emd} \cdot \left|\frac{1}{n} - \frac{1}{\|\hbs\|_1}\right| \\
&\leq (n + \zeta) \cdot \left(\frac{1}{n} - \frac{1}{n - \zeta}\right) \\
&\leq \frac{1}{n} \cdot \frac{\zeta(n + \zeta)}{n - \zeta} \\
&\leq \frac{3\zeta}{n},
\end{align*}
where the last inequality follows our assumption that $\zeta \leq n / 2$.

As a result, from the triangle inequality, we have
\begin{align*}
\|\ba - \hba\|_{\emd}
& \leq \|\ba - \hbs/n\|_{\emd} + \|\hbs/n - \hba\|_{\emd} \\
& \leq \frac{\zeta}{n} + \frac{3\zeta}{n} = \frac{4\zeta}{n},
\end{align*}
concluding our proof.
\end{proof}

\subsubsection{Reducing $\ell_1$ to EMD: Proof of \Cref{lem:final-guarantee-deterministic}}

In this section we go from the recovery guarantee under $\ell_1$ metric to that under EMD; to do this, we need the following two statements from prior work. 
%
\begin{lemma}[Model-Alignment of EMD with $\cM_w$~\cite{indyk2011k}] \label{lem:model-alignment}
For any $\bx \in \R_{\geq 0}^{G_\Delta}, k \in \N$ and $\eta \in (0, 1)$, there exist $w = O(k / \eta^2)$ and $\by^* \in \cM_w$ such that $\|\by^* - \bP\bs\|_1 \leq \eta \cdot \min_{k\text{-sparse } \bx'} \|\bx - \bx'\|_{\emd}.$
\end{lemma}

\begin{lemma}[EMD-to-$\ell_1$ Expansion~\cite{indyk2003fast}] \label{lem:emd-to-l1-expansion}
For all $\bz \in \R^{G_{\Delta}}$, $\|\bz\|_{\emd} \leq \|\bP\bz\|_1.$
\end{lemma}
%

\begin{proof}[Proof of \Cref{lem:final-guarantee-deterministic}]
Recall that we use $\bs$ to denote the true sum $\sum_{i=1}^n \bp_i$. We set $\eta = \eta' / 6$ and let $w = O(k/\eta^2) = O(k/(\eta')^2)$ be as in \Cref{lem:model-alignment}, which ensures that there exists $\by^* \in \cM_w$ with
\begin{align} \label{eq:tmp1}
\|\by^* - \bP\bs\|_1 \leq \eta \cdot \min_{k\text{-sparse } \bs'} \|\bs - \bs'\|_{\emd}.
\end{align}
Thus, using \Cref{lem:emd-to-l1-expansion}, we can derive
\begin{align*}
\|\bs - \bs^*\|_{\emd} &\leq \|\bP(\bs - \bs^*)\|_1 \\
(\text{triangle inequality}) &\leq \|\hby - \bP\bs\|_1 + \|\hby - \bP\bs^*\|_1 \\
(\text{how } \bs^* \text{ is computed}) &\leq 2\|\hby - \bP\bs\|_1 \\
(\text{\Cref{lem:l1-recovery-tree}}) &\leq 6\|\by^* - \bP\bs\|_1 \\
& \quad + O\left(\sum_{i \in [\ell]} \frac{1}{2^i} \left\|\bnu_i|_{V_i \cup S_i}\right\|_1\right) \\
&\overset{\eqref{eq:tmp1}}{\leq} \eta' \cdot \min_{k\text{-sparse } \bs'} \|\bs - \bs'\|_{\emd} \\
& \quad + O\left(\sum_{i \in [\ell]} \frac{1}{2^i} \left\|\bnu_i|_{V_i \cup S_i}\right\|_1\right). \qedhere
\end{align*}
\iffalse
% the following is the original (uncompressed) version.
From \Cref{lem:l1-recovery-tree}, we have
\begin{align} \label{eq:tmp2}
\|\hby - \bP\bs\|_1 \leq 3\|\by^* - \bP\bs\|_1 + 3\left(\sum_{i \in [\ell]} \left\|\bnu_i|_{V_i \cup S_i}\right\|_1\right).
\end{align}
Due to the linear program we solve in Line~\ref{line:lp}, we have
\begin{align} \label{eq:tmp3}
\|\hby - \bP\bs^*\|_1 \leq \|\hby - \bP\bs\|_1.
\end{align}
Combining the inequalities \eqref{eq:tmp1}--\eqref{eq:tmp3}, we arrive at
\begin{align*}
\|\bP(\bs - \bs^*)\|_1 &\leq \|\by^* - \bP\bs\|_1 + \|\hby - \bP\bs^*\|_1 \\
&\overset{\eqref{eq:tmp3}}{\leq} \|\by^* - \bP\bs\|_1 + \|\hby - \bP\bs\|_1 \\
&\overset{\eqref{eq:tmp2}}{\leq} 4\|\by^* - \bP\bs\|_1 + 3\left(\sum_{i \in [\ell]} \frac{1}{2^i} \left\|\bnu_i|_{V_i \cup S_i}\right\|_1\right) \\
&\overset{\eqref{eq:tmp1}}{\leq} \eta' \cdot \min_{k\text{-sparse } \bs'} \|\bs - \bs'\|_{\emd} + 3\left(\sum_{i \in [\ell]} \frac{1}{2^i} \left\|\bnu_i|_{V_i \cup S_i}\right\|_1\right),
\end{align*}
where the first inequality follows from the triangle inequality. 

Finally, by appealing to \Cref{lem:emd-to-l1-expansion}, we can conclude the proof
\begin{align*}
\|\bs - \bs^*\|_{\emd} \leq \eta' \cdot \min_{k\text{-sparse } \bs'} \|\bs - \bs'\|_{\emd} + 3\left(\sum_{i \in [\ell]} \left\|\bnu_i|_{V_i \cup S_i}\right\|_1\right).
\qquad 
\qedhere
\end{align*}
\fi
\end{proof}

\subsection{Proof of \Cref{lem:l1-recovery-tree}}
\begin{proof}[Proof of \Cref{lem:l1-recovery-tree}]
%We write $S$ as a shorthand for $S_0 \cup \cdots \cup S_\ell$ and $\by$ as a shorthand for $[\by_0 \cdots \by_\ell]$. 
For every $q \in T^* \setminus S$, let $R(q)$ be the highest ancestor of $q$ that does not belong to $S$. We have
\begin{align}
\|\by^*|_{\bar{S}}\|_1 
&= \sum_{q \in T^* \setminus S} \by^*(q) 
= \sum_{i \in [\ell]} \sum_{p \in V_i} \sum_{q \in R^{-1}(p)} \by^*(q) \nonumber \\
& \leq \sum_{i \in [\ell]} \sum_{p \in V_i} 2\by^*(p) 
= 2 \sum_{i \in [\ell]} \by^*(V_i), \label{eq:expand-decay}
\end{align}
where the inequality follows from the second property of $\cM_w$.

Next, consider the algorithm at the $i$th iteration and $p \in V_i$. Since $p$ was not picked, the following must hold for all $q \in S_i \setminus T^*_i$:
%
$\by'(p) \leq \by'(q)$.
%
Observe also that from $|S_i| = \max\{w, |C_{2^i}|\}$ and $|T^*_i| \leq \max\{w, |C_{2^i}|\}$, we also have $|S_i \setminus T^*_i| \geq |T^*_i \setminus S_i| = |V_i|$. Thus, we get
\begin{align} \label{eq:dropped-each-level}
\by'(V_i) \leq \by'(S_i \setminus T^*_i).
\end{align}

From this and~\eqref{eq:expand-decay}, we can further derive
\begin{align}
\|\by^*|_{\bar{S}}\|_1
&\overset{\eqref{eq:expand-decay}}{\leq} 2 \left(\sum_{i \in [\ell]} (\by^*(V_i) - \bP\bs(V_i)) + \bP\bs(S_i \setminus T^*_i) \right) \nonumber \\ &\qquad 
+ \left(\sum_{i \in [\ell]} \bP\bs(V_i) - \bP\bs(\left(S_i \setminus T^*_i\right))\right) \nonumber \\
%\text{(From } \supp(\by^*) \subseteq T^*) 
&\overset{(\square)}{\leq} 2\|\by^* - \bP\bs\|_1 + 2 \left(\sum_{i \in [\ell]} \bP\bs(V_i) - \bP\bs(\left(S_i \setminus T^*_i\right))\right) \nonumber \\
%\text{(From definition of } \by') 
&\overset{(\bigtriangleup)}{\leq} 2\|\by^* - \bP\bs\|_1 + 2 \left(\sum_{i \in [\ell]} \frac{1}{2^i} \left\|\bnu_i|_{V_i \cup \left(S_i \setminus T^*_i\right)}\right\|_1\right) \nonumber \\ &\qquad
+ 2\left(\sum_{i \in [\ell]} \by'(V_i) - \by'(\left(S_i \setminus T^*_i\right))\right) \nonumber \\
%&= 2\|\by^* - \bP\bs\|_1 - 2 \left(\sum_{i \in [\ell]} \frac{1}{2^i} \bnu_i(V_i)\right) + 2\left(\sum_{i \in [\ell]} \by'_i(V_i)\right) \\
& \overset{\eqref{eq:dropped-each-level}}{\leq} 2\|\by^* - \bP\bs\|_1 + 2 \left(\sum_{i \in [\ell]} \frac{1}{2^i} \left\|\bnu_i|_{V_i \cup \left(S_i \setminus T^*_i\right)}\right\|_1\right), \label{eq:optimal-norm-outside} 
\end{align}
where $(\square)$ follows from $\supp(\by^*) \subseteq T^* = \bigcup_{i \in [\ell]} T^*_i$ and $(\bigtriangleup)$ follows from how $\by'$ is calculated.
\iffalse
% the following is old derivation, which is both space-consuming and gives worse bound.
From this and~\eqref{eq:expand-decay}, we can further derive
\begin{align*}
\|\by^*|_{\bar{S}}\|_1
&\overset{\eqref{eq:expand-decay}}{\leq} 2 \left(\sum_{i \in [\ell]} (\by^*(V_i) - \bP\bs(V_i)) + \bP\bs(V_i)\right) \\
&\leq 2\|\by^* - \bP\bs\|_1 + 2 \sum_{i \in [\ell]} \bP\bs(V_i) \\
\text{(From how } \by' \text{ is calculated)} &= 2\|\by^* - \bP\bs\|_1 + 2\left(\sum_{i \in [\ell]} \left(\by'_i(V_i) - \frac{1}{2^i} \bnu_i(V_i)\right)\right) \\
%&= 2\|\by^* - \bP\bs\|_1 - 2 \left(\sum_{i \in [\ell]} \frac{1}{2^i} \bnu_i(V_i)\right) + 2\left(\sum_{i \in [\ell]} \by'_i(V_i)\right) \\
& \overset{\eqref{eq:dropped-each-level}}{\leq} 2\|\by^* - \bP\bs\|_1 - 2 \left(\sum_{i \in [\ell]} \frac{1}{2^i} \bnu_i(V_i)\right) + 2\left(\sum_{i \in [\ell]} \by'_i(S_i \setminus T^*_i)\right). 
\end{align*}
We can then bound the last term by
\begin{align*}
\sum_{i \in [\ell]} \by_i(S_i \setminus T^*_i) &= \sum_{i \in [\ell]} \bP\bs(S_i \setminus T^*_i) + \sum_{i \in [\ell]} (\by_i(S_i \setminus T^*_i) - \bP\bs(S_i \setminus T^*_i)) \\
&\leq \|\by^* - \bP\bs\|_1 + \sum_{i \in [\ell]} \frac{1}{2^i} \bnu_i(S_i \setminus T^*_i).
\end{align*}
Combining the two, we get
\begin{align}
\|\by^*|_{\bar{S}}\|_1 \leq 4\|\by^* - \bP\bs\|_1 + 2 \left(\sum_{i \in [\ell]} \frac{1}{2^i} \left\|\bnu_i|_{V_i \cup \left(S_i \setminus T^*_i\right)}\right\|_1\right). \label{eq:optimal-norm-outside}
\end{align}
\fi
%
Finally, notice that
\begin{align*}
& \|\hby - \bP\bs\|_1 
= \|\by'|_{S} - \bP\bs|_{S}\|_1 + \|\bP\bs_{\bar{S}}\|_1 \\
%&= \left(\sum_{i \in [\ell]} \frac{1}{2^i} \|\bnu_i|_{S_i}\|_1\right) + \|\bP\bs|_{\bar{S}}\|_1 \\
&\leq \left(\sum_{i \in [\ell]} \frac{1}{2^i} \|\bnu_i|_{S_i}\|_1\right) + \|\by^*|_{\bar{S}}\|_1 + \|\by^*|_{\bar{S}} - \bP\bs|_{\bar{S}}\|_1 \\
&\overset{\eqref{eq:optimal-norm-outside}}{\leq} \left(\sum_{i \in [\ell]} \frac{1}{2^i} \|\bnu_i|_{S_i}\|_1\right) \\
& \qquad + \left(2\|\by^* - \bP\bs\|_1 + 2 \left(\sum_{i \in [\ell]} \frac{1}{2^i} \left\|\bnu_i|_{V_i \cup \left(S_i \setminus T^*_i\right)}\right\|_1\right)\right) \\
& \qquad + \|\by^* - \bP\bs\|_1 \\
&\leq 3\|\by^* - \bP\bs\|_1 + 3\left(\sum_{i \in [\ell]} \frac{1}{2^i} \left\|\bnu_i|_{V_i \cup S_i}\right\|_1\right),
\end{align*}
where the first two steps follow from $\hby = \by'|_S$ and how each entry of $\by'$ is computed.
\end{proof}
